Deep Convolutional Neural Network and Transfer Learning for Locomotion Intent Prediction

Powered prosthetic legs must anticipate the user's intent when switching between different locomotion modes (e.g., level walking, stair ascent/descent, ramp ascent/descent). Numerous data-driven classification techniques have demonstrated promising results for predicting user intent, but the performance of these intent prediction models on novel subjects remains undesirable. In other domains (e.g., image classification), transfer learning has improved classification accuracy by using previously learned features from a large dataset (i.e., pre-trained models) and then transferring this learned model to a new task where a smaller dataset is available. In this paper, we develop a deep convolutional neural network with intra-subject (subject-dependent) and inter-subject (subject-independent) validations based on a human locomotion dataset. We then apply transfer learning for the subject-independent model using a small portion (10%) of the data from the left-out subject. We compare the performance of these three models. Our results indicate that the transfer learning (TL) model outperforms the subject-independent (IND) model and is comparable to the subject-dependent (DEP) model (DEP Error: 0.74 $\pm$ 0.002%, IND Error: 11.59 $\pm$ 0.076%, TL Error: 3.57 $\pm$ 0.02% with 10% data). Moreover, as expected, transfer learning accuracy increases with the availability of more data from the left-out subject. We also evaluate the performance of the intent prediction system in various sensor configurations that may be available in a prosthetic leg application. Our results suggest that a thigh IMU on the the prosthesis is sufficient to predict locomotion intent in practice.

==> method.tex <==
Supposing the input influence matrix $\mathcal{G}_k$ in output trajectory tracking control law \eqref{FTScontroller}  is unknown, we can formulate a constrained optimization problem to design the control input $u_k$ and the input influence matrix $\mathcal{G}_k$ concurrently. The finite-time stable tracking control law can be formulated as an equality constraints of a min norm controller:

\begin{equation}
    \begin{array}{c}
    \underset{\mathcal{G}_k, u_k}{\min} \|u_k\|_2^2 + w \|\mathcal{G}_k\|^2_{F} \\
    \mathcal{G}_k u_k=f_k \\
    % u_k \in \mathcal{U}, \mathcal{G}_k \in \mathcal{G} \\
    u_{\min} \le u_k \le u_{\max}, \\
    \|\mathcal{G}_{k} - \mathcal{G}_{k-1}\|_F\le L\|y_{k} - y_{k-1}\| \\
    sign(\mathcal{G}_{k}^{i,j})=s_{i,j}
    \end{array}
\end{equation}
where $w$ is a small positive weight to prevent $G_k$ from going to $0$. $u_{\min}$ and $u_{\max}$ are the lower and upper bounds of the control input. We also constrain the $\mathcal{G}_k$ to be Lipschitz continuous. Note that constraints on the sign of $\mathcal{G}_k$ is necessary. If we replace $\mathcal{G}_k$ with $-\mathcal{G}_k$, $-u_k$ then becomes the solution, which may not regulate the tracking error but amplifying it. 

TODO: We have to estimate the bounds of the tracking error here.
